Contractible complexes and non-positive immersions

We provide examples of contractible complexes which fail to have non-positive immersions and weak non-positive immersions, answering a conjecture of Wise in the negative.

==> diagrams/X_skeleton.tex <==
\begin{tikzpicture}[->, thick, main/.style = {draw, circle}] 
\node[main] (1) {$v$}; 
\draw (1) to [out=50,in=310,looseness=12] node[midway, right] {$b$} (1);
\draw (1) to [out=130,in=230,looseness=12] node[midway, left] {$a$} (1);
\end{tikzpicture}

==> links/linkv.tex <==
\begin{tikzpicture}[node distance={10mm and 20mm}, thick, main/.style = {draw, circle, minimum size=1pt, inner sep=2pt}] 
\node[main] (1) {$a$}; 
\node[main] (2) [right=of 1] {$b$}; 
\node[main] (3) [below=of 1] {$\bar{a}$}; 
\node[main] (4) [right=of 3] {$\bar{b}$}; 

\path
    (1) edge[bend left=10] (2)
    (1) edge[bend left=10] (4)
    (2) edge (4)
    (2) edge[bend right=10] (3)
    (3) edge[bend right=10] (4);

\path[magenta]
    (1) edge (3)
    (1) edge[bend right=10] (2)
    (2) edge[bend left=10] (3)
    (1) edge[bend right=10] (4)
    (3) edge[bend left=10] (4);

\end{tikzpicture}

==> links/linkv1.tex <==
\begin{tikzpicture}[node distance={10mm and 20mm}, thick, main/.style = {draw, circle, minimum size=1pt, inner sep=2pt}] 
\node[main] (1) {$e_8$}; 
\node[main] (2) [right=of 1] {$\bar{e_4}$}; 
\node[main] (3) [below=of 1] {$e_1$}; 
\node[main] (4) [right=of 3] {$\bar{e_5}$}; 

\path
    (1) edge (2)
    (1) edge[bend left=10] (4)
    (2) edge (4)
    (3) edge[bend left=10] (2)
    (3) edge (4);

\path[magenta]
    (1) edge[bend right=10] (4)
    (3) edge[bend right=10] (2);

\end{tikzpicture}

==> links/linkv2.tex <==
\begin{tikzpicture}[node distance={10mm and 20mm}, thick, main/.style = {draw, circle, minimum size=1pt, inner sep=2pt}] 
\node[main] (1) {$e_7$}; 
\node[main] (2) [right=of 1] {$e_3$}; 
\node[main] (3) [below=of 1] {$\bar{e_8}$}; 
\node[main] (4) [right=of 3] {$e_4$}; 

\path
    (1) edge[bend left=10] (2)
    (2) edge (4)
    (3) edge (2)
    (3) edge[bend right=10] (4);

\path[magenta]
    (1) edge[bend right=10] (2)
    (3) edge[bend left=10] (4);

\end{tikzpicture}

==> links/linkv3.tex <==
\begin{tikzpicture}[node distance={10mm and 20mm}, thick, main/.style = {draw, circle, minimum size=1pt, inner sep=2pt}] 
\node[main] (1) {$e_2$}; 
\node[main] (2) [right=of 1] {$e_5$}; 
\node[main] (3) [below=of 1] {$\bar{e_7}$}; 
\node[main] (4) [right=of 3] {$\bar{e_3}$}; 

\path
    (1) edge[bend left=10] (2)
    (2) edge[bend right=10] (3)
    (2) edge (4)
    (3) edge (4);

\path[magenta]
    (1) edge[bend right=10] (2)
    (2) edge[bend left=10] (3)
    (1) edge (4);

\end{tikzpicture}

==> links/linkv4.tex <==
\begin{tikzpicture}[node distance={10mm and 20mm}, thick, main/.style = {draw, circle, minimum size=1pt, inner sep=2pt}] 
\node[main] (1) {$\bar{e_1}$}; 
\node[main] (2) [right=of 1] {$\bar{e_6}$}; 
\node[main] (3) [below=of 1] {$\bar{e_2}$}; 
\node[main] (4) [right=of 3] {$e_6$}; 

\path
    (1) edge (2)
    (1) edge (4)
    (2) edge (4)
    (2) edge[bend right=10] (3)
    (3) edge[bend right=10] (4);

\path[magenta]
    (1) edge (3)
    (2) edge[bend left=10] (3)
    (3) edge[bend left=10] (4);

\end{tikzpicture}

==> steps/step0/step0.tex <==
\begin{tikzpicture}[node distance={25mm}, thick, main/.style = {draw, circle}] 
\node (skeleton) at (7.75,0) {
    \scalebox{0.65}{
        \input{steps/step0/step0skeleton}
    }
};
\node (faces) at (0, 0) {
    \scalebox{0.65}{
        \input{steps/step0/step0faces}
    }
};

\draw[->] (faces) to (skeleton);

\end{tikzpicture}

==> steps/step0/step0faces.tex <==
\begin{tikzpicture}[node distance=25mm and 28mm]
    \node (f1) [
        blue,
        draw=none,
        minimum size=1.5cm,
        regular polygon, regular polygon sides=5,
    ]{};

    \draw[->-] (f1.corner 1) -- (f1.corner 2) node[midway, above left] {$e_2$};
    \draw[->-] (f1.corner 2) -- (f1.corner 3) node[midway, left] {$e_{3}$};
    \draw[->-] (f1.corner 3) -- (f1.corner 4) node[midway, below] {$e_{4}$};
    \draw[->-] (f1.corner 4) -- (f1.corner 5) node[midway, right] {$e_{5}$};
    \draw[->-] (f1.corner 5) -- (f1.corner 1) node[midway, above right] {$e_{1}$};
    
\end{tikzpicture}

==> steps/step0/step0skeleton.tex <==
\begin{tikzpicture}[->,node distance={25mm}, thick, main/.style = {draw, circle}, minimum size=8mm, font=\small]

\node (f1) [
        blue,
        draw=none,
        minimum size=3cm,
        regular polygon, regular polygon sides=5,
        shape border rotate=18,
    ]{};

\node[main] (5) at (f1.corner 1) {$v_2$};
\node[main] (1) at (f1.corner 2) {$v_1$};
\node[main] (2) at (f1.corner 3) {$v_5$};
\node[main] (11) at (f1.corner 4) {$v_4$};
\node[main] (7) at (f1.corner 5) {$v_3$};

% First loop
\path[every node/.style={font=\small\sffamily}]
    (5) edge node[above] {$e_2$} (7)
    (7) edge node[right] {$e_3$} (11)
    (1) edge node [left, pos=.7] {$e_1$} (5)
    (2) edge node [left, pos=.3] {$e_5$} (1)
    (11) edge node [below, pos=.4] {$e_4$} (2);

\end{tikzpicture}

==> steps/step1/step1.tex <==
\begin{tikzpicture}[node distance={25mm}, thick, main/.style = {draw, circle}] 
\node (skeleton) at (7.75,0) {
    \scalebox{0.65}{
        \input{steps/step1/step1skeleton}
    }
};
\node (faces) at (0, 0) {
    \scalebox{0.65}{
        \input{steps/step1/step1faces}
    }
};

\draw[->] (faces) to (skeleton);

\end{tikzpicture}

==> steps/step1/step1faces.tex <==
\begin{tikzpicture}[node distance=25mm and 28mm]
    \node (f1) [
        blue,
        draw=none,
        minimum size=1.5cm,
        regular polygon, regular polygon sides=5,
    ]{};

    \draw[->-] (f1.corner 1) -- (f1.corner 2) node[midway, above left] {$e_2$};
    \draw[->-] (f1.corner 2) -- (f1.corner 3) node[midway, left] {$e_{3}$};
    \draw[->-] (f1.corner 3) -- (f1.corner 4) node[midway, below] {$e_{4}$};
    \draw[->-] (f1.corner 4) -- (f1.corner 5) node[midway, right] {$e_{5}$};
    \draw[->-] (f1.corner 5) -- (f1.corner 1) node[midway, above right] {$e_{1}$};
    
    \node (f2) [
        draw=none,
        minimum size=1.5cm,
        regular polygon, regular polygon sides=5,
        right of=f1,
    ]{};
    
    \draw[->-] (f2.corner 1) -- (f2.corner 2) node[midway, above left] {$e_8$};
    \draw[->-] (f2.corner 2) -- (f2.corner 3) node[midway, left] {$e_{9}$};
    \draw[->-] (f2.corner 3) -- (f2.corner 4) node[midway, below] {$e_{3}$};
    \draw[->-] (f2.corner 4) -- (f2.corner 5) node[midway, right] {$e_{6}$};
    \draw[->-] (f2.corner 5) -- (f2.corner 1) node[midway, above right] {$e_{7}$};
    
\end{tikzpicture}

==> steps/step1/step1skeleton.tex <==
\begin{tikzpicture}[->,node distance={25mm}, thick, main/.style = {draw, circle}, minimum size=8mm, font=\small]

\node (f1) [
        blue,
        draw=none,
        minimum size=3cm,
        regular polygon, regular polygon sides=5,
        shape border rotate=18,
    ]{};

\node (f2) [
        blue,
        draw=none,
        minimum size=3cm,
        regular polygon, regular polygon sides=5,
        anchor=corner 3,
        shape border rotate=-90,
    ] at (f1.corner 5) {};

\node[main] (5) at (f1.corner 1) {$v_2$};
\node[main] (1) at (f1.corner 2) {$v_1$};
\node[main] (2) at (f1.corner 3) {$v_5$};
\node[main] (11) at (f1.corner 4) {$v_4$};
\node[main] (7) at (f1.corner 5) {$v_3$};

\node[main] (9) at (f2.corner 5) {$v_6$};
\node[main] (6) at (f2.corner 1) {$v_7$};
\node[main] (4) at (f2.corner 2) {$v_8$};

% First loop
\path[every node/.style={font=\small\sffamily}]
    (4) edge node [above, pos=.7] {$e_9$} (7)
    (9) edge node [right, pos=.3] {$e_7$} (6)
    (6) edge node [right, pos=.7] {$e_8$} (4)
    (7) edge node[right] {$e_3$} (11);

% Third loop
\path[every node/.style={font=\small\sffamily}]
    (1) edge node [left, pos=.7] {$e_1$} (5)
    (2) edge node [left, pos=.3] {$e_5$} (1)
    (11) edge node [below, pos=.4] {$e_4$} (2)
    (11) edge node [below, pos=.4] {$e_6$} (9);

% Extra edges
\draw[<-] (7) -- node[above] {$e_3$} (5);

\end{tikzpicture}

==> steps/step2/step2.tex <==
\begin{tikzpicture}[node distance={25mm}, thick, main/.style = {draw, circle}] 
\node (skeleton) at (7.75,0) {
    \scalebox{0.65}{
        \input{steps/step2/step2skeleton}
    }
};
\node (faces) at (0, 0) {
    \scalebox{0.65}{
        \input{steps/step2/step2faces}
    }
};

\draw[->] (faces) to (skeleton);

\end{tikzpicture}

==> steps/step2/step2faces.tex <==
\begin{tikzpicture}[node distance=25mm and 28mm]
    \node (f1) [
        blue,
        draw=none,
        minimum size=1.5cm,
        regular polygon, regular polygon sides=5,
    ]{};

    \draw[->-] (f1.corner 1) -- (f1.corner 2) node[midway, above left] {$e_2$};
    \draw[->-] (f1.corner 2) -- (f1.corner 3) node[midway, left] {$e_{3}$};
    \draw[->-] (f1.corner 3) -- (f1.corner 4) node[midway, below] {$e_{4}$};
    \draw[->-] (f1.corner 4) -- (f1.corner 5) node[midway, right] {$e_{5}$};
    \draw[->-] (f1.corner 5) -- (f1.corner 1) node[midway, above right] {$e_{1}$};
    
    \node (f2) [
        draw=none,
        minimum size=1.5cm,
        regular polygon, regular polygon sides=5,
        right of=f1,
    ]{};
    
    \draw[->-] (f2.corner 1) -- (f2.corner 2) node[midway, above left] {$e_8$};
    \draw[->-] (f2.corner 2) -- (f2.corner 3) node[midway, left] {$e_{9}$};
    \draw[->-] (f2.corner 3) -- (f2.corner 4) node[midway, below] {$e_{3}$};
    \draw[->-] (f2.corner 4) -- (f2.corner 5) node[midway, right] {$e_{6}$};
    \draw[->-] (f2.corner 5) -- (f2.corner 1) node[midway, above right] {$e_{7}$};
    
    \node (f3) [
        draw=none,
        minimum size=1.5cm,
        regular polygon, regular polygon sides=5,
        right of=f2,
    ]{};
    
    \draw[->-] (f3.corner 1) -- (f3.corner 2) node[midway, above left] {$e_{4}$};
    \draw[->-] (f3.corner 2) -- (f3.corner 3) node[midway, left] {$e_5$};
    \draw[->-] (f3.corner 3) -- (f3.corner 4) node[midway, below] {$e_{1}$};
    \draw[->-] (f3.corner 4) -- (f3.corner 5) node[midway, right] {$e_{10}$};
    \draw[->-] (f3.corner 5) -- (f3.corner 1) node[midway, above right] {$e_{6}^{-1}$};
    
\end{tikzpicture}

==> steps/step2/step2skeleton.tex <==
\begin{tikzpicture}[->,node distance={25mm}, thick, main/.style = {draw, circle}, minimum size=8mm, font=\small]
\node[main] (7) at (7.25,1) {$v_3$}; 
\node[main] (4) at (5.75,1) {$v_8$};

\node[main] (5) at (8.75,1) {$v_2$};

\node[main] (6) at (7.25,-1) {$v_7$};
\node[main] (9) at (8.75,-1) {$v_6$};

\node[main] (1) at (10.5,1) {$v_1$};
\node[main] (2) at (12,1) {$v_5$};
\node[main] (11) at (12,-1) {$v_4$};

% First loop
\path[every node/.style={font=\small\sffamily}]
    (4) edge node [above] {$e_9$} (7);

% Second loop
\path[every node/.style={font=\small\sffamily}]
    (5) edge[bend left=0] node [right] {$e_{10}$} (9)
    (9) edge node [above] {$e_7$} (6)
    (6) edge[bend left=20] node [above, pos=0.4] {$e_8$} (4);

% Third loop
\path[every node/.style={font=\small\sffamily}]
    (1) edge node [above] {$e_1$} (5)
    (2) edge node [above] {$e_5$} (1)
    (11) edge node [right] {$e_4$} (2)
    (11) edge node [below] {$e_6$} (9);

% Extra edges
\draw[<-] (7) -- node[above] {$e_2$} (5);
\draw[rounded corners=5mm] (7) -- +(0,1) -- +(5.75,1) -- node[right] {$e_3$} +(5.75,-2) -- (11);

\end{tikzpicture}

==> steps/step3/step3.tex <==
\begin{tikzpicture}[node distance={25mm}, thick, main/.style = {draw, circle}] 
\node (skeleton) at (7.75,0) {
    \scalebox{0.65}{
        \input{steps/step3/step3skeleton}
    }
};
\node (faces) at (0, 0) {
    \scalebox{0.65}{
        \input{steps/step3/step3faces}
    }
};

\draw[->] (faces) to (skeleton);

\end{tikzpicture}

==> steps/step3/step3faces.tex <==
\begin{tikzpicture}[node distance=25mm and 28mm]
    \node (f1) [
        blue,
        draw=none,
        minimum size=1.5cm,
        regular polygon, regular polygon sides=5,
    ]{};

    \draw[->-] (f1.corner 1) -- (f1.corner 2) node[midway, above left] {$e_2$};
    \draw[->-] (f1.corner 2) -- (f1.corner 3) node[midway, left] {$e_{3}$};
    \draw[->-] (f1.corner 3) -- (f1.corner 4) node[midway, below] {$e_{4}$};
    \draw[->-] (f1.corner 4) -- (f1.corner 5) node[midway, right] {$e_{5}$};
    \draw[->-] (f1.corner 5) -- (f1.corner 1) node[midway, above right] {$e_{1}$};
    
    \node (f2) [
        draw=none,
        minimum size=1.5cm,
        regular polygon, regular polygon sides=5,
        right of=f1,
    ]{};
    
    \draw[->-] (f2.corner 1) -- (f2.corner 2) node[midway, above left] {$e_8$};
    \draw[->-] (f2.corner 2) -- (f2.corner 3) node[midway, left] {$e_{9}$};
    \draw[->-] (f2.corner 3) -- (f2.corner 4) node[midway, below] {$e_{3}$};
    \draw[->-] (f2.corner 4) -- (f2.corner 5) node[midway, right] {$e_{6}$};
    \draw[->-] (f2.corner 5) -- (f2.corner 1) node[midway, above right] {$e_{7}$};
    
    \node (f3) [
        draw=none,
        minimum size=1.5cm,
        regular polygon, regular polygon sides=5,
        right of=f2,
    ]{};
    
    \draw[->-] (f3.corner 1) -- (f3.corner 2) node[midway, above left] {$e_{4}$};
    \draw[->-] (f3.corner 2) -- (f3.corner 3) node[midway, left] {$e_5$};
    \draw[->-] (f3.corner 3) -- (f3.corner 4) node[midway, below] {$e_{1}$};
    \draw[->-] (f3.corner 4) -- (f3.corner 5) node[midway, right] {$e_{10}$};
    \draw[->-] (f3.corner 5) -- (f3.corner 1) node[midway, above right] {$e_{6}^{-1}$};
    
    \node (f4) [
        draw=none,
        minimum size=1.5cm,
        regular polygon, regular polygon sides=5,
        below of=f1
    ] {};
    
    \draw[->-] (f4.corner 1) -- (f4.corner 2) node[midway, above left] {$e_{9}$};
    \draw[->-] (f4.corner 2) -- (f4.corner 3) node[midway, left] {$e_2^{-1}$};
    \draw[->-] (f4.corner 3) -- (f4.corner 4) node[midway, below] {$e_{11}$};
    \draw[->-] (f4.corner 4) -- (f4.corner 5) node[midway, right] {$e_{12}$};
    \draw[->-] (f4.corner 5) -- (f4.corner 1) node[midway, above right] {$e_{13}$};
    
\end{tikzpicture}

==> steps/step3/step3skeleton.tex <==
\begin{tikzpicture}[->,node distance={25mm}, thick, main/.style = {draw, circle}, minimum size=8mm, font=\small]
\node[main] (7) at (0,0) {$v_3$}; 
\node[main] (4) at (4.5,0) {$v_8$};

\node[main] (8) at (5.75,1) {$v_{10}$};
\node[main] (0) at (7.25,1) {$v_9$};
\node[main] (5) at (8.75,1) {$v_2$};

\node[main] (6) at (7.25,-1) {$v_7$};
\node[main] (9) at (8.75,-1) {$v_6$};

\node[main] (1) at (10.5,1) {$v_1$};
\node[main] (2) at (12,1) {$v_5$};
\node[main] (11) at (12,-1) {$v_4$};

% First loop
\path[every node/.style={font=\small\sffamily}]
    (4) edge[bend left=45] node [above] {$e_9$} (7);

% Second loop
\path[every node/.style={font=\small\sffamily}]
    (8) edge[bend right=20] node [above, pos=0.9] {$e_{13}$} (4)
    (0) edge node [above] {$e_{12}$} (8)
    (5) edge node [above] {$e_{11}$} (0)
    (5) edge[bend left=0] node [right] {$e_{10}$} (9)
    (9) edge node [above] {$e_7$} (6)
    (6) edge[bend left=20] node [above, pos=0.4] {$e_8$} (4);

% Third loop
\path[every node/.style={font=\small\sffamily}]
    (1) edge node [above] {$e_1$} (5)
    (2) edge node [above] {$e_5$} (1)
    (11) edge node [right] {$e_4$} (2)
    (11) edge node [below] {$e_6$} (9);

% Extra edges
\draw[<-,rounded corners=5mm] (7) -- +(0,2)-| node[above, pos=.25] {$e_2$} (5);
\draw[rounded corners=5mm] (7) -- +(0,-2)-| node[below, pos=.25] {$e_3$} (11);

\end{tikzpicture}

==> steps/step4/step4.tex <==
\begin{tikzpicture}[node distance={25mm}, thick, main/.style = {draw, circle}] 
\node (skeleton) at (7.75,0) {
    \scalebox{0.65}{
        \input{steps/step4/step4skeleton}
    }
};
\node (faces) at (0, 0) {
    \scalebox{0.65}{
        \input{steps/step4/step4faces}
    }
};

\draw[->] (faces) to (skeleton);

\end{tikzpicture}

==> steps/step4/step4faces.tex <==
\begin{tikzpicture}[node distance=25mm and 28mm]
    \node (f1) [
        blue,
        draw=none,
        minimum size=1.5cm,
        regular polygon, regular polygon sides=5,
    ]{};

    \draw[->-] (f1.corner 1) -- (f1.corner 2) node[midway, above left] {$e_2$};
    \draw[->-] (f1.corner 2) -- (f1.corner 3) node[midway, left] {$e_{3}$};
    \draw[->-] (f1.corner 3) -- (f1.corner 4) node[midway, below] {$e_{4}$};
    \draw[->-] (f1.corner 4) -- (f1.corner 5) node[midway, right] {$e_{5}$};
    \draw[->-] (f1.corner 5) -- (f1.corner 1) node[midway, above right] {$e_{1}$};
    
    \node (f2) [
        draw=none,
        minimum size=1.5cm,
        regular polygon, regular polygon sides=5,
        right of=f1,
    ]{};
    
    \draw[->-] (f2.corner 1) -- (f2.corner 2) node[midway, above left] {$e_8$};
    \draw[->-] (f2.corner 2) -- (f2.corner 3) node[midway, left] {$e_{9}$};
    \draw[->-] (f2.corner 3) -- (f2.corner 4) node[midway, below] {$e_{3}$};
    \draw[->-] (f2.corner 4) -- (f2.corner 5) node[midway, right] {$e_{6}$};
    \draw[->-] (f2.corner 5) -- (f2.corner 1) node[midway, above right] {$e_{7}$};
    
    \node (f3) [
        draw=none,
        minimum size=1.5cm,
        regular polygon, regular polygon sides=5,
        right of=f2,
    ]{};
    
    \draw[->-] (f3.corner 1) -- (f3.corner 2) node[midway, above left] {$e_{4}$};
    \draw[->-] (f3.corner 2) -- (f3.corner 3) node[midway, left] {$e_5$};
    \draw[->-] (f3.corner 3) -- (f3.corner 4) node[midway, below] {$e_{1}$};
    \draw[->-] (f3.corner 4) -- (f3.corner 5) node[midway, right] {$e_{10}$};
    \draw[->-] (f3.corner 5) -- (f3.corner 1) node[midway, above right] {$e_{6}^{-1}$};
    
    \node (f4) [
        draw=none,
        minimum size=1.5cm,
        regular polygon, regular polygon sides=5,
        below of=f1
    ] {};
    
    \draw[->-] (f4.corner 1) -- (f4.corner 2) node[midway, above left] {$e_{9}$};
    \draw[->-] (f4.corner 2) -- (f4.corner 3) node[midway, left] {$e_2^{-1}$};
    \draw[->-] (f4.corner 3) -- (f4.corner 4) node[midway, below] {$e_{11}$};
    \draw[->-] (f4.corner 4) -- (f4.corner 5) node[midway, right] {$e_{12}$};
    \draw[->-] (f4.corner 5) -- (f4.corner 1) node[midway, above right] {$e_{13}$};
    
    \node (f5) [
        draw=none,
        minimum size=1.5cm,
        regular polygon, regular polygon sides=5,
        right of=f4
    ] {};
    
    \draw[->-] (f5.corner 1) -- (f5.corner 2) node[midway, above left] {$e_{16}$};
    \draw[->-] (f5.corner 2) -- (f5.corner 3) node[midway, left] {$e_{17}$};
    \draw[->-] (f5.corner 3) -- (f5.corner 4) node[midway, below] {$e_{9}^{-1}$};
    \draw[->-] (f5.corner 4) -- (f5.corner 5) node[midway, right] {$e_{14}$};
    \draw[->-] (f5.corner 5) -- (f5.corner 1) node[midway, above right] {$e_{15}$};
    
\end{tikzpicture}

==> steps/step4/step4skeleton.tex <==
\begin{tikzpicture}[->,node distance={25mm}, thick, main/.style = {draw, circle}, minimum size=8mm, font=\small]
\node[main] (7) at (0,0) {$v_3$}; 
\node[main] (3) at (1,1) {$v_{13}$};
\node[main] (13) at (2.25,1) {$v_{12}$};
\node[main] (10) at (3.5,1) {$v_{11}$};
\node[main] (4) at (4.5,0) {$v_8$};

\node[main] (8) at (5.75,1) {$v_{10}$};
\node[main] (0) at (7.25,1) {$v_9$};
\node[main] (5) at (8.75,1) {$v_2$};

\node[main] (6) at (7.25,-1) {$v_7$};
\node[main] (9) at (8.75,-1) {$v_6$};

\node[main] (1) at (10.5,1) {$v_1$};
\node[main] (2) at (12,1) {$v_5$};
\node[main] (11) at (12,-1) {$v_4$};

% First loop
\path[every node/.style={font=\small\sffamily}]
    (3) edge[bend right=20] node [above, pos=0.9] {$e_{17}$} (7)
    (13) edge node [above] {$e_{16}$} (3)
    (10) edge node [above] {$e_{15}$} (13)
    (4) edge[bend right=20] node [above, pos=0.1] {$e_{14}$} (10)
    (4) edge[bend left=45] node [above] {$e_9$} (7);

% Second loop
\path[every node/.style={font=\small\sffamily}]
    (8) edge[bend right=20] node [above, pos=0.9] {$e_{13}$} (4)
    (0) edge node [above] {$e_{12}$} (8)
    (5) edge node [above] {$e_{11}$} (0)
    (5) edge[bend left=0] node [right] {$e_{10}$} (9)
    (9) edge node [above] {$e_7$} (6)
    (6) edge[bend left=20] node [above, pos=0.4] {$e_8$} (4);

% Third loop
\path[every node/.style={font=\small\sffamily}]
    (1) edge node [above] {$e_1$} (5)
    (2) edge node [above] {$e_5$} (1)
    (11) edge node [right] {$e_4$} (2)
    (11) edge node [below] {$e_6$} (9);

% Extra edges
\draw[<-,rounded corners=5mm] (7) -- +(0,2)-| node[above, pos=.25] {$e_2$} (5);
\draw[rounded corners=5mm] (7) -- +(0,-2)-| node[below, pos=.25] {$e_3$} (11);

\end{tikzpicture}

==> steps/step5/step5.tex <==
\begin{tikzpicture}[node distance={25mm}, thick, main/.style = {draw, circle}] 
\node (skeleton) at (7.75,0) {
    \scalebox{0.65}{
        \input{steps/step5/step5skeleton}
    }
};
\node (faces) at (0, 0) {
    \scalebox{0.65}{
        \input{steps/step5/step5faces}
    }
};

\draw[->] (faces) to (skeleton);

\end{tikzpicture}

==> steps/step5/step5faces.tex <==
\begin{tikzpicture}[node distance=25mm and 28mm]
    \node (f1) [
        blue,
        draw=none,
        minimum size=1.5cm,
        regular polygon, regular polygon sides=5,
    ]{};

    \draw[->-] (f1.corner 1) -- (f1.corner 2) node[midway, above left] {$e_2$};
    \draw[->-] (f1.corner 2) -- (f1.corner 3) node[midway, left] {$e_{3}$};
    \draw[->-] (f1.corner 3) -- (f1.corner 4) node[midway, below] {$e_{4}$};
    \draw[->-] (f1.corner 4) -- (f1.corner 5) node[midway, right] {$e_{5}$};
    \draw[->-] (f1.corner 5) -- (f1.corner 1) node[midway, above right] {$e_{1}$};
    
    \node (f2) [
        draw=none,
        minimum size=1.5cm,
        regular polygon, regular polygon sides=5,
        right of=f1,
    ]{};
    
    \draw[->-] (f2.corner 1) -- (f2.corner 2) node[midway, above left] {$e_8$};
    \draw[->-] (f2.corner 2) -- (f2.corner 3) node[midway, left] {$e_{9}$};
    \draw[->-] (f2.corner 3) -- (f2.corner 4) node[midway, below] {$e_{3}$};
    \draw[->-] (f2.corner 4) -- (f2.corner 5) node[midway, right] {$e_{6}$};
    \draw[->-] (f2.corner 5) -- (f2.corner 1) node[midway, above right] {$e_{7}$};
    
    \node (f3) [
        draw=none,
        minimum size=1.5cm,
        regular polygon, regular polygon sides=5,
        right of=f2,
    ]{};
    
    \draw[->-] (f3.corner 1) -- (f3.corner 2) node[midway, above left] {$e_{4}$};
    \draw[->-] (f3.corner 2) -- (f3.corner 3) node[midway, left] {$e_5$};
    \draw[->-] (f3.corner 3) -- (f3.corner 4) node[midway, below] {$e_{1}$};
    \draw[->-] (f3.corner 4) -- (f3.corner 5) node[midway, right] {$e_{10}$};
    \draw[->-] (f3.corner 5) -- (f3.corner 1) node[midway, above right] {$e_{6}^{-1}$};
    
    \node (f4) [
        draw=none,
        minimum size=1.5cm,
        regular polygon, regular polygon sides=5,
        below of=f1
    ] {};
    
    \draw[->-] (f4.corner 1) -- (f4.corner 2) node[midway, above left] {$e_{9}$};
    \draw[->-] (f4.corner 2) -- (f4.corner 3) node[midway, left] {$e_2^{-1}$};
    \draw[->-] (f4.corner 3) -- (f4.corner 4) node[midway, below] {$e_{11}$};
    \draw[->-] (f4.corner 4) -- (f4.corner 5) node[midway, right] {$e_{12}$};
    \draw[->-] (f4.corner 5) -- (f4.corner 1) node[midway, above right] {$e_{13}$};
    
    \node (f5) [
        draw=none,
        minimum size=1.5cm,
        regular polygon, regular polygon sides=5,
        right of=f4
    ] {};
    
    \draw[->-] (f5.corner 1) -- (f5.corner 2) node[midway, above left] {$e_{16}$};
    \draw[->-] (f5.corner 2) -- (f5.corner 3) node[midway, left] {$e_{17}$};
    \draw[->-] (f5.corner 3) -- (f5.corner 4) node[midway, below] {$e_{9}^{-1}$};
    \draw[->-] (f5.corner 4) -- (f5.corner 5) node[midway, right] {$e_{14}$};
    \draw[->-] (f5.corner 5) -- (f5.corner 1) node[midway, above right] {$e_{15}$};
    
    \node (f6) [
        draw=none,
        minimum size=1.5cm,
        regular polygon, regular polygon sides=5,
        right of=f5
    ] {};
    
    \draw[->-] (f6.corner 1) -- (f6.corner 2) node[midway, above left] {$e_{19}$};
    \draw[->-] (f6.corner 2) -- (f6.corner 3) node[midway, left] {$e_{20}$};
    \draw[->-] (f6.corner 3) -- (f6.corner 4) node[midway, below] {$e_{3}^{-1}$};
    \draw[->-] (f6.corner 4) -- (f6.corner 5) node[midway, right] {$e_2^{-1}$};
    \draw[->-] (f6.corner 5) -- (f6.corner 1) node[midway, above right] {$e_{10}$};
    
\end{tikzpicture}

==> steps/step5/step5skeleton.tex <==
\begin{tikzpicture}[->,node distance={25mm}, thick, main/.style = {draw, circle}, minimum size=8mm, font=\small]
\node[main] (7) at (0,0) {$v_3$}; 
\node[main] (3) at (1,1) {$v_{13}$};
\node[main] (13) at (2.25,1) {$v_{12}$};
\node[main] (10) at (3.5,1) {$v_{11}$};
\node[main] (4) at (4.5,0) {$v_8$};

\node[main] (8) at (5.75,1) {$v_{10}$};
\node[main] (0) at (7.25,1) {$v_9$};
\node[main] (5) at (8.75,1) {$v_2$};

\node[main] (6) at (7.25,-1) {$v_7$};
\node[main] (9) at (8.75,-1) {$v_6$};

\node[main] (1) at (10.5,1) {$v_1$};
\node[main] (2) at (12,1) {$v_5$};
\node[main] (11) at (12,-1) {$v_4$};
\node[main] (12) at (10.5,-1) {$v_{14}$};

% First loop
\path[every node/.style={font=\small\sffamily}]
    (3) edge[bend right=20] node [above, pos=0.9] {$e_{17}$} (7)
    (13) edge node [above] {$e_{16}$} (3)
    (10) edge node [above] {$e_{15}$} (13)
    (4) edge[bend right=20] node [above, pos=0.1] {$e_{14}$} (10)
    (4) edge[bend left=45] node [above] {$e_9$} (7);

% Second loop
\path[every node/.style={font=\small\sffamily}]
    (8) edge[bend right=20] node [above, pos=0.9] {$e_{13}$} (4)
    (0) edge node [above] {$e_{12}$} (8)
    (5) edge node [above] {$e_{11}$} (0)
    (5) edge[bend left=0] node [right] {$e_{10}$} (9)
    (9) edge node [above] {$e_7$} (6)
    (6) edge[bend left=20] node [above, pos=0.4] {$e_8$} (4);

% Third loop
\path[every node/.style={font=\small\sffamily}]
    (1) edge node [above] {$e_1$} (5)
    (2) edge node [above] {$e_5$} (1)
    (11) edge node [right] {$e_4$} (2)
    (12) edge node [below] {$e_{20}$} (11)
    (9) edge node [below] {$e_{19}$} (12);

% Extra edges
\path[every node/.style={font=\small\sffamily}]
    (11) edge[bend right=30] node [above] {$e_{18}$} (9);
\draw[<-,rounded corners=5mm] (7) -- +(0,2)-| node[above, pos=.25] {$e_2$} (5);
\draw[rounded corners=5mm] (7) -- +(0,-2)-| node[below, pos=.25] {$e_3$} (11);

\end{tikzpicture}
